PAWS: Paraphrase Adversaries from Word Scrambling

Existing paraphrase identification datasets lack sentence pairs that have high lexical overlap without being paraphrases. Models trained on such data fail to distinguish pairs like flights from New York to Florida and flights from Florida to New York. This paper introduces PAWS (Paraphrase Adversaries from Word Scrambling), a new dataset with 108,463 well-formed paraphrase and non-paraphrase pairs with high lexical overlap. Challenging pairs are generated by controlled word swapping and back translation, followed by fluency and paraphrase judgments by human raters. State-of-the-art models trained on existing datasets have dismal performance on PAWS (<40% accuracy); however, including PAWS training data for these models improves their accuracy to 85% while maintaining performance on existing tasks. In contrast, models that do not capture non-local contextual information fail even with PAWS training examples. As such, PAWS provides an effective instrument for driving further progress on models that better exploit structure, context, and pairwise comparisons.

==> experiment_wiki.tex <==
\section{Experiments on Wiki-WS} \label{sec:experiment_wiki}

\textbf{this section could be ``Use WS as a Standalone Dataset''. WS dataset may have a label balance issue or data size issue. This section discuss a possible solution for that.}

This section shows experiments on Wikipedia. This shows a use case when we don't have standard dataset in the Wikipedia domain and we have imbalanced labels.

\subsection{Extension Method}

Describe how we use back-translation to generate paraphrase pairs. Then we can combine it with WS data to create a new dataset. Shall we call it Wiki-WS++?

\subsection{Experiments on Annotated Data}

Describe how much data we have human annotations. Provide some statistics. The experiment settings include

Model: BOW, bi-LSTM, ESIM, DecAtt, DIIN, BERT

Training data: Wiki-WS++

Testing data: Wiki-WS test

Is available, show some aggregate statistics on wins/losses of different models. E.g., calculate the token distance of the change (to see if one model is better at local reordering vs longer changes).

\subsection{Experiments on Noisy Data}

We have high negative rates on WS and high positive rates on back-translation. We can use them as noisy data and optionally do fine tuning.


The result table can be merged with the one above.
